Technical Challenges in Maintaining Tax Prep Software with Large Language Models

As the US tax law evolves to adapt to ever-changing politico-economic realities, tax preparation software plays a significant role in helping taxpayers navigate these complexities. The dynamic nature of tax regulations poses a significant challenge to accurately and timely maintaining tax software artifacts. The state-of-the-art in maintaining tax prep software is time-consuming and error-prone as it involves manual code analysis combined with an expert interpretation of tax law amendments. We posit that the rigor and formality of tax amendment language, as expressed in IRS publications, makes it amenable to automatic translation to executable specifications (code). Our research efforts focus on identifying, understanding, and tackling technical challenges in leveraging Large Language Models (LLMs), such as ChatGPT and Llama, to faithfully extract code differentials from IRS publications and automatically integrate them with the prior version of the code to automate tax prep software maintenance.

==> Sections/objectives.tex <==
% \vspace{0.5 em}
\section{Objectives.}
The core objective of this project is to evaluate the {\bf efficacy} and {\bf trustworthiness} of pre-trained large language models, such as ChatGPT, in updating tax software to comply with new tax legislation as outlined by IRS publications.
This investigation seeks to determine the capability of AI to autonomously reformulate software code,
ensuring that it is following the amended tax regulations, thereby providing a measure of the
practical applicability of AI in the domain of tax software administration.


==> Sections/table_old.tex <==
\begin{table}[!tbh]
    \centering
\caption{Preliminary Results. \textbf{TBC}: Tax Bracket Calculations,
\textbf{EITC}: Earned Income Tax Credit,
\textbf{SD}: Standard deductions of the elderly and blind,
\textbf{I}: Income,
\textbf{A}: Age,
\textbf{FS}: Filing Status,
\textbf{\#C}: Number of children,
\textbf{D}: Disability,
\textbf{S}: Single,
\textbf{MFJ}: Married Filing Jointly.
}
    \label{tab:my_label}
    \resizebox{0.8\textwidth}{!}{%
    \begin{tabular}{| c | c | c | c | c | c | c | }
    \hline
    %\rule{0pt}{25pt}
     \textbf{Domain} & \textbf{AI Prompts} & \textbf{Tax Law} & \textbf{\makecell{Prior Software} }& \textbf{\makecell{Outcome}} \\ 
     \hline 
     %\rule{0pt}{25pt}
       \makecell{Tax Brackets \\ (2020)} & \makecell{Generate Code for TBC \\ (S)} & Not Given & Not Given & \makecell{Correct except for \\  tax rates 35$\%$+37$\%$}\\
    \hline
        \makecell{Tax Brackets \\ (2020)} & \makecell{Generate Code for TBC \\ (S+MFJ)} & Not Given & Not Given &\makecell{Correct except for \\ tax rates 35$\%$+37$\%$}\\
    \hline
        \makecell{Tax Brackets \\ (2021)} & \makecell{Generate Code for TBC \\ (S)} & Not Given  & Given (2020) & Correct \\
    \hline
        \makecell{Tax Brackets \\ (2021)} & \makecell{Generate Code for TBC  \\ (S+MFJ)} & Not Given & Given (2020) & Correct \\
    \hline
        \makecell{Tax Brackets \\ (2021)} & \makecell{Generate Code for TBC \\ (S+MFJ+SD)} &  Given & Not Given & Correct \\
    \hline     
        \makecell{EITC (2020)} & \makecell{Generate Code for EITC \\ based on (I, A, FS, \#C, D)} & Not Given & Not Given & \makecell{Failed on cut-offs \\ and for single (S)}\\
    \hline
        EITC (2020) &  \makecell{Generate Code for EITC \\ based on (I, A, FS, \#C, D)} & Given & Not Given & \makecell{Correct} \\
    \hline
        EITC (2021) & \makecell{Generate Code for EITC \\ based on (I, A, FS, \#C, D)} & Not Given & Given & \makecell{Failed on cut-offs \\ and credit amounts}\\
  
    \hline
    \end{tabular}
    }
\end{table}
